On Bayesian Mechanics: A Physics of and by Beliefs

The aim of this paper is to introduce a field of study that has emerged over the last decade called Bayesian mechanics. Bayesian mechanics is a probabilistic mechanics, comprising tools that enable us to model systems endowed with a particular partition (i.e., into particles), where the internal states (or the trajectories of internal states) of a particular system encode the parameters of beliefs about external states (or their trajectories). These tools allow us to write down mechanical theories for systems that look as if they are estimating posterior probability distributions over the causes of their sensory states. This provides a formal language for modelling the constraints, forces, potentials, and other quantities determining the dynamics of such systems, especially as they entail dynamics on a space of beliefs (i.e., on a statistical manifold). Here, we will review the state of the art in the literature on the free energy principle, distinguishing between three ways in which Bayesian mechanics has been applied to particular systems (i.e., path-tracking, mode-tracking, and mode-matching). We go on to examine a duality between the free energy principle and the constrained maximum entropy principle, both of which lie at the heart of Bayesian mechanics, and discuss its implications.

==> content/cuts.tex <==
CUTS

...

It is interesting to note that action potentials can be modelled as the same sorts of topological excitations that we call instantons in gauge theories \cite{ori2022}: just like we model \emph{virtual} particles, such as phonons, as topological excitations in condensed matter theory, this suggests that approximate Bayesian inference as a gauge theory is no mathematical artefact but has some actual explanatory power. 

In closing, we believe that new results in the foundations of Bayesian mechanics that have recently become available afford us the opportunity to `reboot' the free energy principle literature, at least insofar as how we speak about, and how we think about its relation to other principles in physics and how they are used in science. These results demonstrate the duality of the FEP to the principle of (constrained) maximum entropy and establish robust connections to other core mathematical principles and technologies in theoretical physics (e.g., gauge theory) and statistics (e.g., information geometry). 


a description known as \emph{active inference} \cite{friston_active_2015,friston_active_2017,friston2009reinforcement,da_costa_active_2020,tschantz_reinforcement_2020}. Such a description provides an alternative perspective to standard views in reinforcement learning that explain action as maximizing a scalar reward function \cite{sutton2018reinforcement,silver2021reward}. Mathematically, these views can be reconciled to some extent if the notion of hard constraints can be relaxed to softer penalties and reward or utility functions can be related to `desired' probability densities through a logarithmic transform \cite{levine2018reinforcement,millidge_understanding_2021,millidge2021applications,da_costa_relationship_2020}. However, framing the behaviour of particular systems in terms of Bayesian mechanics offers some interesting insights. For example, in reinforcement learning, self-organisation is traditionally described in terms of a function of certain states or outcomes (i.e., a reward, cost, or loss function). Conversely, in Bayesian mechanics, self-organisation is described in terms of functionals (i.e., functions of functions); namely, functions of probabilistic beliefs. This has the striking consequence that, in Bayesian mechanics, self-organisation depends upon what a particular system believes about external states of affairs, not merely on (reward, cost, loss) functions of those states. In short, Bayesian mechanics provides a formulation to think about the constraints and goals that govern particular systems; especially those, like biological organisms, which must maintain homeostatic bounds. The relationship between maximising entropy, which produces exponentiated constraint functions, and optimal control of allostatic or existential variables can be seen as an instance of Todorov duality \cite{todorov_general_2008}.

In fact,  concerns about the falsifiability 
It is therefore a threefold category mistake to say that principles (like the FEP) are unfalsifiable or unverifiable. On the one hand, principles like the FEP are simply not the kind of that can be subject to falsification: they are mathematical statements that are verifiable by construction, in the sense that they are mathematically consistent (as we saw the example of stationary action in section \ref{sec:preliminaries}). On the other hand, it is an \textit{empirical} question whether some principle provides an apt explanation of some physical phenomena; and that \textit{empirical application} is a verifiable fact.  
Finally, it bears mentioning that from the point of view of contemporary philosophy of science, concerns about falsifiability are arguably a hangover from 20th century epistemology. We have inherited these concerns from the Popperian model of science\textemdash wherein we can demarcate science from pseudoscience via critical experiments, leading to the confirmation/falsification of individual theories. This view was arguably only ever a gloss on the actual practice of science, and was rejected even by followers of Popper, such as Lakatos \cite{lakatos1976falsification}. 

At a conceptual level, the fibre bundle picture of the CMEP licenses a "bag of tricks" or "swiss army knife" interpretation of complex systems: that the organising principles of complex self-organising systems are no different than the simple physical rules of other much simpler systems, and that complexity emerges from many simple systems doing "unintelligent" things together, like simply following geodesics on a constraint geometry. Indeed, as has been mentioned previously \cite{Sakthivadivel2022b}, the maximum entropy formulation of the FEP has no process-level details\textemdash and more generally, the implementation of free energy minimisation is a free variable in any theory to which the FEP couples. It may be that complexity emerges from a system of interacting subsystems doing unintelligent things which together maintain system-ness; this stable configuration of the system is then selected for, under the tautological interpretation of a system, understood as necessarily being stable enough to be the kind of system that it is. Indeed, natural selection needs no intelligent designer: order emerges from simple tautologies, and a confluence of simple lower-level dynamical systems. %also talk about funnel stuff Ken brought up here !

The idea that a complex system, and in particular the brain, are simply a "bag of tricks" consisting of things that work for given purposes, with no organising principles at all, has been put forth by others as well \cite{rama, dennet, buckner, clements, adami, levin-cog}. The geometric viewpoint of the FEP/CMEP duality suggests a framework in which to investigate how the dynamics of lower-level processes are shaped by simple geodesics in the state space, and features of complexity emerge from "less intelligent" actions at a lower level.

...

The broad scope of the FEP also gains some clarity in light of the above, and in light of the emergence of Bayesian mechanics as a field. A field of inquiry has emerged around the FEP and related approaches. With hindsight, it has become clear that the FEP itself is not a scientific theory per se, and should not be presented as such, but instead a principle and ensuing method, which has the same kind of status and role in theory construction as the principle of least action or the principle of maximum entropy. As such, the FEP is one among a pantheon of core mathematical principles that underwrite physics, and Bayesian mechanics in particular. While this lack of clarity has been detrimental, more charitably, one might view this confusion as an expression of growing pains of what is arguably emerging as a new field of inquiry.

% \dars{flagging: may need to handle this example more pedagogically}

% For a worked example of where this hierarchy comes from, consider the Dirac equation for a free fermion field,\footnote{By free, we mean uncoupled to a gauge field. By fermion field, we mean a field whose quanta are particles 1) obeying Fermi-Dirac statistics, and 2) comprising matter. An example is an electron.}
% \begin{equation}\label{dirac-equation}
% (i\hbar \gamma^\mu \partial_\mu - mc)\psi = 0.
% \end{equation}
% Here, $\psi$ is the wavefunction of a bispinor, $\psi : \R^{3,1} \to \C^4$. The fact that any such free fermion is described by a wavefunction $\psi : \R^{3,1} \to \C$ is a more general fact of quantum mechanics, and when we take only one component\textemdash specify a particular particle for this field\textemdash we get quantum mechanics back. Then, solving \eqref{dirac-equation} and getting a plane-wave for $\psi$, we can model how particles behave for specific trajectories and initial conditions (a dynamical theory). 

% Returning to the top of the hierarchy, \eqref{dirac-equation} arises from the variation of the action functional
% \[
% \int_\Omega \bar\psi(i\hbar \gamma^\mu \partial_\mu - mc^2)\psi \dd{\text{vol}_\Omega}.
% \]


%ON THE FENCE ABOUT THIS PARAGRAPH (Maxwell really likes this)
% In the 1910s and 1920s, a new sort of physics for particles was devised, which came to be called quantum mechanics. When combined with other data about what a quantum particle was, this boiled down to a collection of rules for the dynamics of quantum particles based primarily in the wavefunction. This mechanical theory comes in some sense from the principle that, for some particle travelling on space-time, any given path is taken with probability proportional to $\exp{\frac{1}{\hbar} S[x(t)]}$.\footnote{This is the path integral approach to quantum mechanics, established by Feynman \cite{RPF}. Other approaches are possible, such as the matrix mechanics approach, which arises from the correspondence principle between classical and quantum energy spectra.} In the late 1920s through the 1930s, it was almost immediately realised that the quantum mechanics of particles was not sufficient to describe the natural world, which is spatially extended. Instead, physics was reformulated in terms of fields \cite{weinberg}.


%\ch{I'm going to leave some feedback here on the section above, but it also ties into some general comments on the thrust of the paper and I guess also Section 6. I don't agree with the definition of Bayesian mechanics written here. In my opinion BM is not something that describes physical systemhood in terms of surprisal and entropy, those concepts are very much prior to the BM-gloss on dynamics that has been added recently. I think Prirogine's work and England's work and the work of many others in complex systems have already worked out a lot of those concepts. You can write down the flow of stationary systems as self-preserving and surprise-minimizing (potential-minimizing) based on decades of earlier work and that doesn't really have any bearing on Bayesian mechanics. The Helmholtz decomposition of SDE flows is also not integral or even important to Bayesian mechanics -- it's just a particular way we can decompose the deterministic part of the flow of an SDE. Bayesian mechanics has the word `Bayesian' in it because it's about probability distributions and particularly posterior probability distributions (i.e. beliefs in the face of uncertainty inherent in sensory states), and the precise conditions under which systems can be thought of as parameterizing beliefs via functions whose domain are quantities that characterize the system (e.g. states, flows, trajectories, other measures). It has the word `mechanics' in it, because there are forces and fields that determine how beliefs move in that space. Interestingly, these belief spaces and the flows along them are also related to the physical mechanics of the system (in ways we don't really understand yet). This new mechanics of beliefs and belief-flows has not been well developed yet in the context of SDEs (although see Eun-jin Kim's work). It has just started with some of the recent FEP literature. But we \textit{do} know a lot about the mathematics and geometry of those statistical spaces (not necessarily the mechanical flows on them though). This knowledge has largely been provided by information geometry}.

%\dars{I think the intro explains this without some of the requisite details, but this (Conor's) view is pretty much in line with the discussions we've been having, I think. It isn't that BMech determines how systems behave, \emph{per se}---classical and statistical mechanics can be written via the FEP, for instance, which would mean we're redefining classical mechanics as the Bayesian mechanics of classical objects, which I don't think is the intention (maybe it is, but this is not how I see it). Instead, BMech is about the beliefs held by the system and how those beliefs evolve, and is manifested by the minimisation of variational FE under the synchronisation map. Dually, however, it is about the probability density the system samples under and how that is enforced or evolved. That this is consistent with previous work by e.g. England is no accident; the point \emph{is} that the dual of the FEP is more traditional, older stuff, like the CMEP. Hence that we can define BMech by looking at this other stuff that people are more accustomed to.}

%\dars{If we come to some consensus on this it might be wise to iterate over the intro again to make that consensus clear}

%\dars{Possibly pointing out how nicely this fits into max cal as well, in discussing probabilities of and on flows being a referent for belief updating in the Bayesian mechanical sense}]

%\ch{Thanks Dalton; these are useful comments and is helping me understand better where everyone's coming from. I have some thoughts about this phrase: "classical and statistical mechanics can be written via the FEP, for instance, which would mean we're redefining classical mechanics as the Bayesian mechanics of classical objects...". I would agree with this completely except for the last part, where you say `we're redefining classical mechanics as the Bayesian mechanics of classical objects...". I think the redefinition of classical and statistical mechanics in terms of minimizing surprisal is the essence of the FEP and the surprise-minimization framework -- the large part of the monograph. But importantly I do not consider this Bayesian mechanics -- Bayesian mechanics is more of a `special corollary' of the FEP that applies in certain cases. For instance, a univariate SDE (some classic 1-D OU process) can be described as minimizing surprise on average. In my opinion, this is not an example of Bayesian mechanics. Maybe others would disagree with me -- in which case I'd be curious to hear that argument.

%As you said later on, "BMech is about the beliefs held by the system and how those beliefs evolve". I think BMech really only applies when we've narrowed down to more specific cases from the general "surprise-minimizing" framework, which applies to all random dynamical systems with a stationary state. For BMech to apply /be interesting we need 1) a multivariate system, IMO with internal and blanket states (although this is my unsubstantiated opinion as of now) and 2) we need a function that takes internal states (or some measure/function/projection thereof, such as the most likely one, given blanket states) and projects them to a space of probability distributions. This is a more specific case than the general message of the FEP, which is more how I would describe what has been said in the introduction (about systemhood, resisting dissipation, minimization of surprisal). So in summary, my general view is that FEP is more general than BayesMech, and BayesMech is just a special case of multipartite systems where the "FE" part of the "FEP" really can be used to tell a story about how systems appear to minimize VFE/ maximize model evidence in face of sensory data, aka approximate Bayesian inference.} 

%\dars{This is great --- to sketch out some thoughts really quickly, I would say BMech is the mechanics of systems that engage in genuine approximate Bayesian inference, i.e., systems that have evolving beliefs --- possibly qualifying that these are controlled systems --- and perhaps we can go narrower and say it defines in particular the image of these systems on a statistical manifold. \\
%\vskip0.5cm
%It's probably important to draw a distinction between genuine ABI and more trivial stuff like dissipating towards a mode; not sure how to handle that but presumably the answer is obvious, and lies in the fact that dissipative systems don't have a true MB. \\
%\vskip0.5cm
%We can define BMech using these dual statements about our beliefs about a system that carries beliefs, but the fact that this returns us from FEP to max ent is important because we want consistency between the two.}

%\dars{Definitely worth airing this out in the intro, else people may miss the point of what defining `Bayesian mechanics' is for. On the other hand, if more internal discussion is needed to come to a consensus, we can always pass this onto a different paper. In the paper I just did I point out in a couple of places that the max ent stuff works best in only trivial regimes where we don't have a genuine Bayesian mechanics, hence `\emph{towards} a geometry and analysis for Bayesian mechanics.' We can propose a definition here but I don't think we'll get to proving anything about it, so might be best to avoid. That is to say, I really see a `genuine' BMech as falling under the purview of max cal, whilst max ent covers mostly trivial cases of what could reasonably be called BMech.}


\subsection{Formalising preferences beyond scalar reward functions}

\section{The foundations of a new mechanics}\label{sec:newmechanics}

\dars{Comment from Beren: While the debate over falsifiability of the FEP is interesting -- and I am not totally sure I agree with you about this principle therefore unfalsifiable view (including that the FEP is just a principle as things like markov blankets etc are highly falsifiable) -- I don't think this is a good place for this. I would move this to the discussion section. We really need this section to be going through the mathematical preliminaries to understand Bayesian mechanics}
\dars{beren: this is not true or at least more subtle. The principle of stationary action is true mathematically -- in that you can always write down some action and some dynamics that minimize it -- but the fact that the dynamics of physical systems can be straightforwardly written as minimizing an action functional is actually a striking empirical fact. It would be very possible to have the laws of physics not be describable in such a way -- or at least if they are have some insanely convoluted action functional as to make it essentially underivable}
\dars{From Conor: I think at some point -- perhaps not here, given the physics focus -- it would be helpful to clarify the difference between this distinction (between principled and mechanical descriptions of dynamics, i.e. Lagrangian vs Newtonian descriptions) and a distinction often used in natural, empirical sciences, between phenomenological vs. mechanistic models of data}



We may or may not think the same way as the pioneers of the field do


Arguably, many proponents in the early literature were (at least a bit) overzealous in their proselytising the approach, and in several key respects over promised on unfinished theoretical work, claiming to have a finished theory when only the fundamentals of a new approach (indeed, what is turning into a new chapter of mechanics) were really available 

Perhaps in part because of these elements of presentation, many critics have not bothered to engage with the material, much to the detriment of the FEP literature itself 



In the literature, the term `FEP' designates both a core modelling principle (on an epistemological par with maximum entropy or stationary action) and a new approach to mechanics.

It is now apparent that, much like quantum mechanics, Bayesian mechanics is a new field of inquiry that may be more or less interestingly applied to various kinds of systems




This may be because this domain of investigation is not a theory, but rather a new branch of investigation in mechanics.

That is, to put it bluntly: the FEP isn't One Theory to Rule them All, in no small part because it isn't properly speaking a theory.




%The system's ontological potential (NESS or constraints) is a way of specifying systemic, allowable states.
%The notion of preferences as constraints provides us with a formal means to define system preferences, moving beyond loose language to a formal theory
%This allows us to overcome current limitations of machine learning and inference \mtk{We need a reference for this}
%\dars{might be too far off to cover just yet. Would be cool to discuss it, but being \emph{too} speculative is counterproductive I think. Maybe it'll work when this paragraph is more fleshed out}
%This formulation of self-organisation using stationary action and related techniques take us away from a 20th century view of optimality, defined in terms of value functions
%Usually the reward $R$ is provided by the environment, and is a scalar function
%However, constraints are on something. If they're applied as potentials on log prior probabilities, the constraint space has be to high dimensional
%So, this formulation leads to proper characterization of phenotypes, namely, a high-dimensional characterization of system's systemness, which cannot be specified with a loss function  
%Indeed, unless R is a free-energy, there is no space in the reward function to define the teleology of the system 
%This moves us back to 19th century appreciation of what counts as good behaviour
%The phenotype is not the NESS density but rather the slow subspace and manifold

\dars{Some really speculative, breezier stuff below that may or may not belong}

This paper is, in some sense, a companion to more recent papers that align themselves explicitly with the tradition of Bayesian mechanics, e.g., \cite{DaCosta2021, Ramstead2021, Sakthivadivel2022b}. %Sakthivadivel (2022a,b) and Da Costa et al. (2022). However, we also aim to offer more than merely a technical overview of Bayesian mechanics, but also a reader-friendly introduction. This is more difficult than it may seem. Bayesian mechanics is fundamentally a highly technical and mathematical field. However, the approach has proven to be of interest to a broad, multidisciplinary readership, some of which is highly nontechnical. There is no avoiding this technicality: it is not optional or accidental. If one wants to engage with Bayesian mechanics, one has to do so technically, in no small part because the core intuitions that drive research in Bayesian mechanics are themselves mathematical. That is, Bayesian mechanics works the way that it does because of how the mathematical structures that it harnesses are constructed, and what properties these constructions entail. Due to the broad based foundations of Bayesian mechanics, which draws from at times disparate mathematical resources, it is sometimes difficult to communicate the formal results of the field---a problem compounded by the at times idiosyncratic notation of earlier (and current) literature. Happily, many of the core results of Bayesian mechanics are graphical and geometrical in nature, which allows us to visualise the constructs and get a more intuitive sense of the underlying mathematical constructions. 

But this paper is not merely a companion that converts proofs into painless reading (relatively speaking). The work contained is, we hope, of independent interest: the paper actually does the work of tying everything together very explicitly to introduce the new field, and provides some context and motivation for the emergence of Bayesian mechanics. 

We discuss the implications of the duality between nonequilibrium steady state potentials under the FEP formulation and the kind of constraints that figure in constrained maximum entropy inference. 

We also discuss the duality of the Helmholtz decomposition of the autonomous flow under the FEP (into dissipative and solenoidal components) and the splitting vector fields that arise in the maximum entropy formulation (into horizontal and vertical components) 

The questions of concern in this paper are: 
What are these constraints and potentials, physically? 
How are the flows and manifolds of the system related to the NESS potential and the decomposed autonomous flows under the FEP? 
How are these manifolds and slows related to the constraints of constrained maximum entropy?
What can we learn from the duality of FEP and MaxEnt?
Why does this matter for the dynamics of inference?


, providing a broad disciplinary context for sundry individual theories of active systems as statistical models, and moving towards a view of agents as gauge field theories




Another secondary aim is to help clarify the mathematical validity and epistemological status of Bayesian mechanics, and the cluster of surrounding concepts, namely, the free-energy principle, especially as these relate to canonical approaches in theoretical physics and statistics, such as the principles of maximum entropy and stationary action
We provide some historical context and argue that the early stages of the development of Bayesian mechanics evince striking parallels to the emergence and early development of quantum mechanics
Arguably, what has happened to the field of Bayesian mechanics in the last half decade echoes the trends of development in mathematical physics of the last century.
In a sense, this represents an attempt to do for biophysics what has already been done for particle physics: namely, to draw everything together rigorously in terms of fundamental mathematical principles


2.3. Some analogies to the history of quantum mechanics

A comparison to the historical emergence of another branch of mechanics is instructive, especially with regards to its reception
Much like the FEP, quantum mechanics was developed originally by physicists, not mathematicians. The general pattern that emerges is that physicists, being less concerned with mathematical consistency than they are with being able to model their data, develop mathematically problematic but unreasonably effective models that mathematicians later sanitise and improve.

In the early 1900s, QM was regarded as unscientific and borderline quackery
By the early 1920s, the opposite was the case
What happened? Maths was cleaned up with new insights into functional analysis (cite… something by Hilbert) and probability theory(? von Neumann? Schrodinger?), followed later  by gauge theory (Yang-Mills, Chern-Simons, BRST), and more recently, category theory (Baez-Dolan, Lurie? Atiyah?)
However, there are still grand mysteries about the mathematical formulation of quantum field theory and its extension to theories of gravity, which means the issue is far from settled even with these mathematical tools

A similar story can be told about Bayesian mechanics and its development 
Bayesian mechanics has its origins in:
Jaynes’ maximum entropy principle 
Variational technologies
Applications of path integral formulations (for later, the citation for this is his thesis on classical LAP fit into QED)
Ecological psychology and wanting to make physics consistent with psychology and neuroscience 
Artificial intelligence: Hinton, Dayan, RL, etc. 
At this stage, more of a family resemblance, and connections between disciplines

A key development in this way of thinking was FEP
FEP emerged from this nexus of theories and in some sense is the resulting of realising that the very same maths applies in all these cases, e.g., log evidence – log p 
FEP version 1: 2006 to 2012, the brain is doing variational inference 
FEP version 2: 2012 to 2019, now focused on MBs and information geometry

Some critical work at the end of the 2010s forces a re-appraisal of the mathematical foundations of Bayesian mechanics.
One core focus of work in the area from 2019 onward is a search for mathematical foundations 
Non Equilibrium physics (Da Costa, Friston, Heins)
Categorification (St Clere Smithe)
Gauge theoretic formulation (Sakthivadivel, Virgo)
Analysis (Biehl et al. 2021)
These developments mirror those in quantum mechanics  






The above distinctions between dynamics, mechanics, field theories, and principles is relevant to modelling controversies in the literature, in the sense that a statistical field theory described by the minimisation of (variational) free energy will not yield a thermodynamics for every system it is given. Issues have been pointed out with physicalist(? non-instrumentalist?) interpretations of the FEP which assert that actual energy flows are being manipulated, in the sense of thermodynamical free energy, rather than informational quantities. 
This arrangement of data allows us to make distinctions, from (literal) first principles, between the consequences of the FEP for different systems: for systems with energy flows, we get thermodynamics; for systems with information flows, we get something more general, but which is directly analogous to energy-based dynamics. In other words, we get the thermodynamics of open systems as strictly a special case of Bayesian mechanics.



5.5. “Local ergodicity” and NESS can be formalised more precisely

Ergodicity: “local ergodicity” can be given a precise meaning by appealing to the constraints against which entropy is maximised
The system essentially will not visit all possible states given constraints 

“Ontological potential” is a key notion here

Weighting on states is not exactly a probability density function

Another thought: the dissipative flow is time-reversible, while the solenoidal flow is not
From Bayesian mechanics (Da Costa et al 2022): “As we can see the time-reversible part affords the stochasticity while the time-irreversible part characterises non-equilibria and the accompanying wandering behaviour that characterises life-like systems” 




New paper on phenotypes 

3.3. From flows to stability analysis: centre manifolds, etc.
(some stuff here should be in 2.2)

We can bring into play concepts from stability analysis and centre manifold theory to better understand this flow
Interestingly, these concepts (stable and unstable manifolds) are usually used to finesse and formalise the notions of attractor and repulsor
This is interesting because the FEP at core is about systems with a pullback attractor  

Using the Jacobian of the system, we decompose the overall state space into three subspaces: stable, unstable, and centre space
Tangent to each of these spaces is an invariant manifold:
Stable, unstable, and centre manifolds
The centre manifold is the collection of those orbits that neither decay nor grow exponentially
When the eigenvalues of the centre space are precisely zero (as opposed to just having a zero real part), then the centre manifold is called a slow manifold


Remark: How can we have a steady state if the dissipative flow goes up the gradient? 
The dissipative flow is exactly counterbalanced by the Wiener process part of the dynamics, deterministic flow goes up, random flow goes everywhere and counterbalance on average 

Applying some concepts from stability analysis, we can recover a centre manifold theoretic interpretation of autonomous flow and its relation to NESS

What is a centre manifold? An invariant manifold is a line in the state space constituting a fixed point of the system. This is a trajectory to which a dynamical system valued in that state space will converge. To address Conor’s question, it is thus (in a way) both – the idea is that this is a submanifold within the state space which happens to be a line, and, that this line is a line-shaped attractor, so a system near it will occupy that line or evolve along it.

A centre manifold is a special sort of invariant manifold. The convergence to a centre manifold is in general exponentially fast. This is usually a computational trick: taking a very complicated nonlinear system, we can reduce it to a much simpler system on a line by taking the leading order terms only. The reason being, small perturbations go away, since the centre manifold is the curve solving the system with a stability condition. (This seems similar in spirit to the method of characteristics in PDE analysis.) Another special invariant manifold is a stable manifold, which is the manifold containing all trajectories that go to zero.

If we consider all the possible initial conditions of a system that conforms to the FEP, then we can perform stability analysis on the system equipped with a NESS density
Most trajectories grow or decay exponentially quickly leading to nonsystemic states (death)
A subset of trajectories are constrained to the slow manifold and remain there 
From Friston et al. (2022), we know that the dissipative flow is the part of the flow that forces the system onto the centre manifold
The solenoidal flow is then a slow flow on the manifold, which realises the synchronisation manifold between internal and external modes
 
To summarise, the presence of the NESS density induces a flow of autonomous states
A fast flow towards the manifold, exactly countered by random fluctuations
A slow flow on the manifold, which couples expected internal and external states (inference) 
There are also paths that decay exponentially quickly or grow exponentially fast that we might want to characterise as well–in terms of non-systemic states 

So, it appears that each component of the flow accounts for some aspect of self-evidencing, as follows
The dissipative flow enforces systemness—it is the ‘self’ part of ‘self-evidencing’
The solenoidal flow reflects the way prior system expectations are corrected by evidence—it is the ‘evidence’ part of ‘self-evidencing’

In summary, the idea is that the dissipative flow (flow towards the centre manifold) maintains 'systemness' while the solenoidal flow…

5.6. Ontological potentials and phenotypes 

In previous work, Friston, Ramstead, and colleagues had identified the NESS density itself with the phenotype of a system that conforms to the FEP. 
But in light of developments in the FEP formalism over the last two years, a more precise interpretation is available.
The new idea is this:
The fact that the dynamics of a random dynamical system have a NESS density–or equivalently, the presence of a set of constraints against which entropy is maximised–means that the paths or trajectories of the system in its state space are weighted according to their “systemness,” that is, whether or not they conform to the system. 
The presence of these potentials or constraints confines the system’s trajectories through its state space to specific regions, the centre subspace, with its centre manifolds

In systems subject to the FEP, there emerges a slow manifold that collects those the trajectories of the system that are compatible with the system’s systemness (as it were)
When the system is at NESS:
The dissipative component of the autonomous flow can be interpreted as a fast flow towards the centre manifold (i.e., towards the region of state space that contains systemic states)
The solenoidal component of the autonomous flow is a slow flow on the manifold. 
This flow underwrites the existence of the synchronisation manifold between expected internal states or internal modes and expected external states or external modes. 

(regarding Elan vital)
I would add some caveats to this section that say there is a very fuzzy gradient at hand (current argument) but that the gradient definitely still exists. It is easy to say a human is a more particular thing than a stone. A few arguments here

- Precariousness is something like the number of, or sensitivity to, constraints, and humans both have more constraints and are more sensitive to them than stones

- Karl's comment and other discussions that suggest the particular partition is quite special

- I think I talk at length about how ABIL only applies to stones quite trivially

- Adam Safron has a whole thing about IWMT in stones where he comes to basically the same conclusion, we can use IIT on stones but it's pretty vacuous

. neither \textit{stationarity} (i.e., that the mode underwriting the dynamics of a system system has stopped evolving) nor a \textit{steady state} density (i.e., that the dynamics of a particular system tend towards a specific modal value or attractor)


$G$-theory is the name we have given to a larger theory of complex adaptive systems that we do not yet understand, but whose existence is strongly suggested by the duality between the FEP and the CMEP, explored here.The name $G$-theory was chosen as an homage to $M$-theory in theoretical physics.\footnote{The reader should note that the `$G$' in $G$-theory does not mean anything specific. If pressed, the authors might say that $G$ stands for `gauge,' or maybe `generalised,' or point out that expected free-energy is often denoted \textbf{G}.} The existence of $M$-theory was first conjectured in the 1990s as a unifying treatment of known string theories \cite{witten1995string}; at the time, it was known that specific versions of string theory were dual to each other, and the idea was that there must exist an underlying theory of which all known string theories were aspects of facets. 

